Eigenspace Restructuring: a Principle of Space and Frequency in Neural Networks

Understanding the fundamental principles behind the massive success of neural networks is one of the most important open questions in deep learning. However, due to the highly complex nature of the problem, progress has been relatively slow. In this note, through the lens of infinite-width networks, a.k.a. neural kernels, we present one such principle resulting from hierarchical localities. It is well-known that the eigenstructure of infinite-width multilayer perceptrons (MLPs) depends solely on the concept frequency, which measures the order of interactions. We show that the topologies from deep convolutional networks (CNNs) restructure the associated eigenspaces into finer subspaces. In addition to frequency, the new structure also depends on the concept space, which measures the spatial distance among nonlinear interaction terms. The resulting fine-grained eigenstructure dramatically improves the network's learnability, empowering them to simultaneously model a much richer class of interactions, including Long-Range-Low-Frequency interactions, Short-Range-High-Frequency interactions, and various interpolations and extrapolations in-between. Additionally, model scaling can improve the resolutions of interpolations and extrapolations and, therefore, the network's learnability. Finally, we prove a sharp characterization of the generalization error for infinite-width CNNs of any depth in the high-dimensional setting. Two corollaries follow: (1) infinite-width deep CNNs can break the curse of dimensionality without losing their expressivity, and (2) scaling improves performance in both the finite and infinite data regimes.

==> tex_zoo/code_block.tex <==
 
\section{ARCHITECTURE SPECIFICATIONS}\label{sec:code}
In this section, we provide more details of the architectures used in the experiments. 
\begin{listing}[htb]
       \begin{minted}{python}
from neural_tangents import stax

def MLP(width=2048, depth=1, W_std=0.5, activation=stax.Rbf()): 
    layers = [] 
    for _ in range(depth): 
        layers += [stax.Dense(width, W_std=W_std), activation]
    layers += [stax.Dense(1)]
    return stax.serial(*layers) 

def CNN(width=512, ksize=4, depth=1, W_std=0.5, activation=stax.Rbf(), readout=stax.Flatten(), 
      act_after_readout=True):
    layers = [] 
    conv_op = stax.Conv(width, (ksize, 1), strides=(ksize, 1), W_std=W_std,  padding='VALID')
    for _ in range(depth): 
        layers += [conv_op, activation]
    layers += [readout]
    if act_after_readout: 
        layers += [stax.Dense(width * 4, W_std=W_std), activation]
    layers += [stax.Dense(1)]
    return stax.serial(*layers)

p = 4 # input shape: (-1, p**4, 1, 1) 
S_MLP = MLP(depth=1) # Shallow MLP 
D_MLP = MLP(depth=4) # Deep MLP 

S_CNN = CNN(ksize=p, depth=1, act_after_readout=False) # Shallow CNN 
# One layer CNN with an additional activation-dense layer 
S_CNN_plus_Act = CNN(ksize=p, depth=1, act_after_readout=True) 
D_CNN = CNN(ksize=p**2, depth=2) # Deep CNN
HR_CNN = CNN(ksize=p, depth=3) # High-resolution CNN
# High-resolution CNN with global average pooling readout 
HR_CNN_GAP = CNN(ksize=p, depth=3, readout=stax.GlobalAvgPool(), act_after_readout=False)
# High-resolution CNN with flattening as readout   
HR_CNN_Flatten = CNN(ksize=p, depth=3, act_after_readout=False) 
\end{minted}
\caption{\textbf{Definitions of MLPs, S-CNN, D-CNN and HR-CNN used in the experiments}. 
 The architectures used in the experiments of Fig.~\ref{fig:learning-eigen-modes} are defined as follows. 
 $\text{MLP}^{\otimes 4}$ = D\_MLP, 
$\text{Conv}(p^2)^{\otimes 2}$ = D\_CNN,
$\text{Conv}(p)^{\otimes 4}$ = HR\_CNN. 
The one layer MLP and one layer CNN used in Fig.~\ref{fig:mlp-2} are S\_MLP and S\_CNN\_plus\_Act, resp. The $\text{Conv}(p)^{\otimes 3}\text{-Flatten}=$ HR\_CNN\_Flatten and $\text{Conv}(p)^{\otimes 3}\text{-GAP}= $ HR\_CNN\_GAP.
}
\label{lst:code-block}
\end{listing}
\newpage 
